Causal Graph Learning via Distributional Invariance of Cause-Effect Relationship

This paper introduces a new framework for recovering causal graphs from observational data, leveraging the observation that the distribution of an effect, conditioned on its causes, remains invariant to changes in the prior distribution of those causes. This insight enables a direct test for potential causal relationships by checking the variance of their corresponding effect-cause conditional distributions across multiple downsampled subsets of the data. These subsets are selected to reflect different prior cause distributions, while preserving the effect-cause conditional relationships. Using this invariance test and exploiting an (empirical) sparsity of most causal graphs, we develop an algorithm that efficiently uncovers causal relationships with quadratic complexity in the number of observational variables, reducing the processing time by up to 25x compared to state-of-the-art methods. Our empirical experiments on a varied benchmark of large-scale datasets show superior or equivalent performance compared to existing works, while achieving enhanced scalability.

==> data_sampling.tex <==
\label{sec:data-sampling}
Invariants work when we intentionally introduce augmentations in the observational data to create multiple environments, so that non-causal relationships exhibit large deviations whereas true causal relationships remain unchanged across these environments. To facilitate such changes, we need to identify the basis of the graph.

\begin{definition}[Basis of a DAG]
    \label{def:basis}
    A basis $\boldsymbol{B}$ of a DAG $G:=\{\boldsymbol{X}, \boldsymbol{E}\}$ is a set of mutually independent variables that all other variables in $G$ depend on at least one variable in the basis. 
    \begin{equation}
    \left\{
        \begin{aligned}
        \label{eq:basis}
            &\boldsymbol{B} \subseteq \boldsymbol{X},\\
            &\forall X_i, X_j \in \boldsymbol{B}: X_i \CI X_j,\\
            &\forall X_k \notin\boldsymbol{B}, \exists X_t \in \boldsymbol{B}: X_t \nCI X_k.
        \end{aligned}
    \right.
    \end{equation}
\end{definition}

Trivially, if we change the marginal distribution of the variables in the basis, all other variables in the graph are affected. By sampling-without-replacement from the original data following a new joint distribution of the basis (i.e., $P(\boldsymbol{B})$), we obtain a sub-dataset, in which non-causal conditional distributions show deviations from ones in the original data. 
The margin of such deviations depend on how we ``intervene" the joint distribution $P(\boldsymbol{B})$. For instance, if we uniformly sample sub-datasets from the original data, then for any arbitrary variables $X_i$ and $X_j$, we expect to have identical conditional distribution $P(X_i|X_j)$ across these sub-datasets, hence unhelpful. 
On the other hand, if we follow a well-designed sampling method that produces sub-datasets where $P(X_i|X_j)$ exhibits large deviations, then we can potentially conclude that $X_j$ is not the cause of $X_i$. 
It is essential to note that sampling from observational data does not create interventional data by nature, therefore, we call this kind of ``intervention" as \textbf{weak intervention} as opposed to conventional intervention.


\subsubsection{Find a maximum-sized Basis}
\label{subsec:find_basis}
A straightforward (and greedy) method is to continually perform legal selection of variables into an empty set until that set satisfies the definition of a basis. However, as per Theorem~\ref{theo:premise}, we need to perform weak interventions on the causes. In other words, we need the basis to match the set of source nodes\footnote{Source nodes (or sources) of a graph are nodes that have no parents.}. Although this is infeasible given only the observational data, we can increase the probability of having sources in our basis, according to the following theorem:

\begin{theorem}
    \label{theo:sources}
    The maximum size of a basis of a graph equals the number of sources in that graph.
\end{theorem}

% \begin{proof}
%     \textbf{By Induction.}\\
%     Let $S(G)\subseteq V$ denote the set of sources in $G:=\{V,E\}$. We have the following predicate
%     $P(n)$: ``Given a DAG $G$ of $n$ $(n \geq 1)$ nodes, we have $|\mathcal{B}(G)| \leq |S(G)|$". \\
%     \textbf{Base case} $P(1)$: Because $G$ has only $1$ node, that node is a source and belongs in $\mathcal{B}$, thus $|\mathcal{B}(G)| = |S(G)|$. Which renders $P(1)$ correct.\\
%     \textbf{Induction step}: Suppose $P(n)$ is correct, we want to prove $P(n+1)$ is also correct. For this we use the following truth: ``there always exists a node $X \in V$ of a DAG $G$ that has no children, i.e., $X$ is a leaf node". Now, we prove $P(n+1)$ by following these steps:\\
%     \underline{First}, we remove the leaf $X$ from graph $G$ to obtain graph $G'$ that has $n$ nodes. By assumption $P(n)$:
%         \[|\mathcal{B}(G')| \leq |S(G')|.\]
%     \underline{Then}, we reconnect $X$ into $G'$ to recreate $G$, there are $2$ cases. One, if $X$ is also a source, then there are no variable in the basis that $X$ is dependent on, because $X$ has no child nodes and no parent nodes! Thus:
%         \begin{align*}
%             |\mathcal{B}(G)| = |\mathcal{B}(G')|&+1 \text{ and }|S(G)| = |S(G')| + 1 \\
%             \to &|\mathcal{B}(G)| \leq |S(G)|.
%         \end{align*}
%     Two, if $X$ is not a source, then either parent nodes of $X$ are in the basis or dependent on at least one of node in the basis (by Definition~\ref{def:basis}). Therefore: 
%         \[|\mathcal{B}(G)| = |\mathcal{B}(G')| \leq |S(G')| = |S(G)|.\]
%     This shows $P(n+1)$ is true, and completes the proof. 
% \end{proof}

The proof of Theorem~\ref{theo:sources} is presented in \textbf{Appendix Section~\ref{supp:proof-sources}}. Theorem~\ref{theo:sources} exactly bounds the number of variables in the basis $\mathcal{B}$ by the number of sources in the graph. This allows us to potentially increase the chances of getting sources into the basis by designing an algorithm that produces a maximum-sized basis. 
% However, note that the set of sources may not be the only maximum sized basis in the graph. 
We devise a greedy method (Algorithm~\ref{algo:find-basis}) that provably produces a maximum-sized basis at the computational cost of $O(d^2)$. Specifically, we define for each variable $X$ a metric called dependence value (denoted as $\eta(X)$), which is the number of other variables that naturally depends on $X$: 
$\eta(X) = \big|\Phi(X)\big|, \ \Phi(X) := \{Y\mid Y \in \boldsymbol{X}\setminus\{X\}: Y \nCI X\}.$
Then, we continually select variables (e.g., $X$) in the ascending order of dependence value, and remove its corresponding dependent variables ($\Phi(X)$) from the selection pool. The procedure stops when the pool is empty.
Algorithm~\ref{algo:find-basis}'s theoretical support and time complexity analysis are presented in \textbf{Appendix Section~\ref{supp:basis}}.
% Interestingly, by analysing the basis-finding algorithm, we can lower-bound the performance of the proposal! 
% \begin{theorem}
%     \label{theo:basis-location}
%     All nodes in the basis lie within the path from the source nodes to the first colliders.
% \end{theorem}
% From this theoretical result, let us form sub-graphs $G_i = (V_i, E_i)$ where $V_i \subseteq V$ consisting of exactly one source $S_i \in V$ and nodes that are (1)~dependent on $S_i$, and (2)~have no collider ancestors. Notice that $|\bigcup_i V_i| \leq |V|$. We then come to the conclusion:
% \begin{theorem}
%     \label{theo:error-upper-bound}
%     Given the sub-graphs $G_i$, and an observational data satisfies Identifiablity, then the number of falsely directed causal relationships is upper-bounded by $\sum_i (|V_i| - 1)$.
% \end{theorem}
% The proof of Theorem~\ref{theo:basis-location},~\ref{theo:error-upper-bound} are deferred to the \textbf{Supplementary Material Section~\ref{supp:basis}}.

% This result gives an insight into the upper-bound performance of the basis-finding algorithm.
% \begin{corollary}
%     Given a graph $G:=(V,E), |V| = d$, we can separate the graph into sub-graphs $G'_i$ ($i=[R]$), each consisting of a source node and the nodes that are dependent on that source node to the first colliders. Then, 
% \end{corollary}


\subsubsection{Perform weak interventions}
\label{subsec:weak_intervene}
As we mentioned ealier, a weak intervention is not a ``real" intervention in its nature. We weakly intervene on a set of variables by sampling a sub-dataset from the original data that follows a particular joint distribution of these variables (which are in the basis). Here we demonstrate the method to create meaningful joint distributions so that sub-datasets we produce benefits the use of invariants for causal identification.

First and foremost, as it turns out, once we sample following a different joint distribution of the basis, we produce a sub-dataset whose volume is proportionally smaller than the original dataset. 
\begin{proposition}[Data volume decay rate]
    \label{prop:volume_decay}
    Let $X_i \in \boldsymbol{B}$ be the variable whose new marginal distribution is used to sample-without-replacement data $D$ to produce $D'$, then:
    % \begin{equation}
        $\frac{|D'|}{|D|} = \min_j \frac{P(X_i = x_j)}{P'(X_i = x_j)},$
    % \end{equation}
    where $P(X_i)$ and $P'(X_i)$ are the marginal distributions of $X_i$ in $D$ and in $D'$, respectively.
\end{proposition}


The proof for this proposition is deferred to \textbf{Appendix Section~\ref{supp:proof-volume-decay}}. Proposition~\ref{prop:volume_decay} implies that the larger the size of the basis, the smaller the sub-data set we produce, if we desire significant changes in term of distribution shift. However, if we choose a new joint distribution $P(\boldsymbol{B})$ of $D'$ that is too similar to that of $D$, then the deviations induced by non-causal relationships would be insignificant. Figure~\ref{fig:useful-region} demonstrates the logicality we encounter: The grey region is too far from the original distribution $P_0(\boldsymbol{B}) := P(\boldsymbol{B})$ \hung{(thus the volume of resultant sub-data sets in this region is too small)} and the orange region surrounding each distribution depicts the space of similarity \hung{(thus the resultant distributions in this region do not make significant contribution to the invariant test)}. The green region is the \textit{desirable} region to find new distributions. According to this logic, we formalize the following dilemma: Let $\{P_j(\boldsymbol{B})\}_{j=1}^K$ be the set of \textit{desirable} joint distributions correspond to the sub-datasets $\{D_j\}_{j=1}^K$, then these \textit{desirable} distributions need to satisfy the following requirements:
\begin{equation}
\label{eq:constraints}
\left\{
\begin{aligned}
    &\mathrm{lie~ in~ the~ region~ satisfying~}\frac{|D_k|}{|D|} \geq \gamma\\
    &\mathrm{distributed~ evenly~ in~ that~ region}
\end{aligned}
\right.
% \frac{|D_k|}{|D|} \geq \gamma \text{  and  } d\big(P_i(\mathcal{B}),P_j(\mathcal{B})\big) \geq \sigma,
\end{equation}
where $\gamma, \sigma > 0$ are constant scalars and $d(\cdot,\cdot)$ is any distance function. Note that even if we can choose several joint distributions that satisfy Requirements~(\ref{eq:constraints}), as depicted in Figure~\ref{fig:useful-region}, these distributions may not be optimal since they do not cover evenly the distribution space which may result in some non-causal distributions that are not affected by weak interventions. Therefore, we also need these distributions to uniformly ``distributed" in the search space. 
\begin{figure}[tb]
    \centering
    \begin{minipage}{0.3\linewidth}
    \centering
        \includegraphics[width=0.98\linewidth]{figs/useful-region-2.eps}
        \caption{\textbf{The useful region.} Each green dot represents a joint distribution of the basis. The green region contains \textit{desirable} distributions.}
        \label{fig:useful-region}
    \end{minipage}
    \hfill
    \begin{minipage}{0.68\linewidth}
    \hfill
        \subfigure[Causal graph]{\includegraphics[width=0.3\linewidth]{figs/plausible-sets-a.eps}}
        \hfill
        \subfigure[Markov blanket]{\includegraphics[width=0.3\linewidth]{figs/plausible-sets-b.eps}}
        \hfill
        \subfigure[Plausible parents]{\includegraphics[width=0.32\linewidth]{figs/plausible-sets-c.eps}}
        \caption{\textbf{Finding plausible parents of $X_6$.} (a) is a sub-graph of the ASIA dataset \citep{scutari2009learning}. (b) emphasizes the Markov blanket of $X_6$ in color green, an undirected edge between two variables indicate they are in the other's Markov blanket. (c) shows that there are only $3$ candidates for $X_6$'s causal parents.}
        \label{fig:plausible_set}
    \end{minipage}
\end{figure}
% \textbf{Strategy:} 
To accomplish this, we first locate the boundary of the region that satisfy the first constraint in Requirements~(\ref{eq:constraints}) (the green region in Figure~\ref{fig:useful-region}). Then, we fill in the space by using the weighted average of the distributions on the boundary. This is possible thanks to the convex property of this region, with regard to the first constraint.

\begin{theorem}[Convex Region]
    \label{theo:convex}
    Let $\mathbb{P}$ denote the space of joint distributions $P_j(\boldsymbol{B})$ that satisfy $|D_j|/|D| \geq \gamma$, then $\forall P_u(\boldsymbol{B}), P_v(\boldsymbol{B}) \in \mathbb{P}, \forall \alpha \in [0,1]$, we have:
    % \begin{equation}
        $\alpha P_u(\boldsymbol{B}) + (1 - \alpha) P_v(\boldsymbol{B}) \in \mathbb{P}.$
    % \end{equation}
\end{theorem}
The proof of Theorem~\ref{theo:convex} and the derivation of boundary joint distributions are deferred to \textbf{Appendix Section~\ref{supp:proof-convex}} and \textbf{\ref{supp:weak_intervention}}, respectively. According to this result, we can generate any number of weak interventional distributions by simply choosing the weights $\{\alpha\}$s.
% \begin{proof}
%     For simplicity, we rewrite $P(\mathcal{B}) \equiv P(X)$ where $X$ is the concatenation vector of all joint distribution vectors of variables in $\mathcal{B}$. We want to prove that:
%     \begin{equation}
%         P_t(X) := \alpha P_u(X) + (1 - \alpha) P_v(X) \in \mathbb{P}.
%     \end{equation}
%     Firstly, because $P_u, P_v \in \mathbb{P}$, we have:
%     \begin{equation}
%         \frac{|D_u|}{|D|} = \min_j \frac{P(x_j)}{P_u(x_j)} \geq \gamma
%         \Rightarrow P(x_j) = \gamma P_u(x_j) + \delta_{uj}, \delta_{uj} \geq 0, \forall j.
%     \end{equation}
%     Similarly, $P(x_j) = \gamma P_v(x_j) + \delta_{vj}, \delta_{vj} \geq 0, \forall j$.
%     Now let us examine:
%     \begin{equation}
%     \label{eq:concex_end}
%         \frac{P(x_j)}{P_t(x_j)} = \frac{\alpha P(x_j) + (1-\alpha) P(x_j)}{\alpha P_u(x_j) + (1-\alpha) P_v(x_j)}\\
%         % &=\frac{\gamma\big(\alpha P_u(x_j) + (1-\alpha)P_v(x_j)\big) + \gamma (\delta_{uj} + \delta_{vj})}{\alpha P_u(x_j) + (1-\alpha)P_v(x_j)}\\
%         = \gamma + \frac{\gamma (\delta_{uj} + \delta_{vj})}{\alpha P_u(x_j) + (1-\alpha)P_v(x_j)},
%     \end{equation}
%     which is a monotonically increasing function on $(\delta_{uj} + \delta_{vj}) \geq 0$. Therefore, the function reaches minimum when $(\delta_{uj} + \delta_{vj}) = 0$. Then, from Equation~\ref{eq:concex_end} we conclude:
%     \begin{equation}
%         \frac{P(x_j)}{P_t(x_j)} \geq \gamma \text{, } \forall j 
%         \Leftrightarrow = \min_j \frac{P(x_j)}{P_t(x_j)} = \frac{|D_t|}{|D|} \geq \gamma \Rightarrow P_t \in \mathbb{P}.
%     \end{equation}
%     This conclusion completes the proof.
% \end{proof}
After having generated a large number of distributions in the useful region, we need to select representative distributions so as to satisfy the second constraint of Requirement~(\ref{eq:constraints}). Intuitively, we leverage the K-means \citep{wu2012advances} algorithm and use the centroids for the final new joint distributions for the basis. To this end, we obtain sub-datasets by sampling following these distributions:
\begin{equation}
    D_j \overset{P_j(\boldsymbol{B})}{\sim} \mathcal{D}, \forall j \in [1,\dots,K],
\end{equation}
where $K$ is the number of centroids, which is also the number of sub-data sets we wish to produce. The time complexity of producing such $K$ sub-data sets is $O(Kd) = O(d)$ \citep{wu2012advances}.
The reader is referred to \textbf{Appendix Section~\ref{supp:weak_intervention}} for more details regarding the generation of weakly interventional sampling distributions.




==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak


==> tab/extreme.tex <==
\begin{table}[]
\begin{tabular}{l|ccccc}
\#Edges    & 600            & 700              & 800             & 900           & 1000          \\ \hline
SCORE      & 902.0 $\pm$ 0.0   & 1188.0 $\pm$ 0.0    & 1481.0 $\pm$ 0.0   & 1616.0 $\pm$ 0.0 & 1714.0 $\pm$ 0.0 \\
DAS     & 721.33 $\pm$ 21.6 & 960.0 $\pm$ 12.33  & 1353.67 $\pm$ 11.39 & 1491.67 $\pm$ 19.08 & 1656.67 $\pm$ 5.81 \\
MLPNotears & 239.0 $\pm$ 19.83 & 562.67 $\pm$ 154.89 & 899.5 $\pm$ 195.02 & 1031.0 $\pm$ 0.0 &               \\
Notears & 374.5 $\pm$ 53.92 & 493.91 $\pm$ 88.91 & 488.2 $\pm$ 27.48   & 596.82 $\pm$ 63.26  & 602.0 $\pm$ 106.68
\end{tabular}
\end{table}

==> tab/related-invariants.tex <==
%\renewcommand{\arraystretch}{1.2}
\begin{table}[h]
\centering
\caption{\textbf{Comparison of existing invariant-based methods.} Invariant Causal Prediction (ICP) and Causal-de-finetti require special methods to generate the data on which they are designed.}
\label{tab:existing-methods}
\vspace{0.2cm}
\begin{tabular}{|l|c|c|c|}
\toprule
\multicolumn{1}{|c|}{\textbf{Baselines}} &
  \textbf{ICP} &
  \textbf{Causal-de-finetti} &
  \textbf{Proposal} \\ \midrule
Invariants &
  \begin{tabular}[c]{@{}c@{}}Weights of SCM\\ $X=\gamma Z + \mu$\end{tabular} &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Independencies\\ $X \CI Y \mid Z$\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Conditional Probability\\ $P(X|Z)$\end{tabular} \\ \midrule
Assumptions &
  Causal Sufficiency &
  \multicolumn{1}{c|}{\begin{tabular}[c]{@{}c@{}}Causal Sufficiency\\ Faithfulness\end{tabular}} &
  \begin{tabular}[c]{@{}c@{}}Causal Sufficiency\\ Faithfulness\end{tabular} \\ \midrule
Data model &
  Linear Gaussian &
  None & None \\ \midrule
Data requirement &
  Interventional datasets &
  \multicolumn{1}{c|}{Exchangeable datasets} &
  None\\
  \bottomrule
\end{tabular}
\end{table}
%\renewcommand{\arraystretch}{1.1}
